Beam-based alignment at the Cooler Synchrotron COSY as a prerequisite for an electric dipole moment measurement

The J\"ulich Electric Dipole moment Investigation (JEDI) collaboration aims at a direct measurement of the Electric Dipole Moment (EDM) of protons and deuterons using a storage ring. The measurement is based on a polarization measurement. In order to reach highest accuracy, one has to know the exact trajectory through the magnets, especially the quadrupoles, to avoid the influence of magnetic fields on the polarization vector. In this paper, the development of a beam-based alignment technique is described that was developed and implemented at the COoler SYnchrotron (COSY) at Forschungszentrum J\"ulich. Well aligned quadrupoles permit one to absolutely calibrate the Beam Position Monitors (BPMs). The method is based on the fact that a particle beam, which does not pass through the center of a quadrupole, experiences a deflection. The precision reached by the method is approximately 40 micro meter. Some consequences for the design of a new high precision storage ring for EDM mesasurements are discussed.

==> authors.tex <==
%Authors
\author{T.~Wagner}
\email[corresponding author: ]{t.wagner@fz-juelich.de}
\affiliation{III. Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{A.~Nass}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{J.~Pretz}
\affiliation{III. Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}
\affiliation{JARA--FAME (Forces and Matter Experiments), Forschungszentrum J\"ulich and RWTH Aachen University, Germany}

%
\author{F.~Abusaif}
\affiliation{III. Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{A.~Aggarwal}
\affiliation{Marian Smoluchowski Institute of Physics, Jagiellonian University, 30348 Cracow, Poland}

\author{A.~Andres}
\affiliation{III. Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{I.~Bekman}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{N.~Canale}
\affiliation{University of Ferrara and INFN, 44100 Ferrara, Italy}

\author{I.~Ciepal}
\affiliation{Institute of Nuclear Physics, Polish Academy of Sciences, 31342 Crakow, Poland}

\author{G.~Ciullo}
\affiliation{University of Ferrara and INFN, 44100 Ferrara, Italy}

\author{F. Dahmen}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{S.~Dymov}
\affiliation{University of Ferrara and INFN, 44100 Ferrara, Italy}
\affiliation{Laboratory of Nuclear Problems, Joint Institute for Nuclear Research, 141980 Dubna, Russia}

\author{C.~Ehrlich}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{R.~Gebel}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{K.~Grigoryev}
\affiliation{III. Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}


\author{D.~Grzonka}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{V.~Hejny}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{J.~Hetzel}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{A.~Kacharava}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{V.~Kamerdzhiev}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{S. Karanth}
\affiliation{Marian Smoluchowski Institute of Physics, Jagiellonian University, 30348 Cracow, Poland}

\author{I.~Keshelashvili}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{A.~Kononov}
\affiliation{University of Ferrara and INFN, 44100 Ferrara, Italy}

\author{A.~Kulikov}
\affiliation{Laboratory of Nuclear Problems, Joint Institute for Nuclear Research, 141980 Dubna, Russia}

\author{K.~Laihem}
\affiliation{III. Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}

\author{A.~Lehrach}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}
\affiliation{JARA--FAME (Forces and Matter Experiments), Forschungszentrum J\"ulich and RWTH Aachen University, Germany}

\author{P.~Lenisa}
\affiliation{University of Ferrara and INFN, 44100 Ferrara, Italy}

\author{N.~Lomidze}
\affiliation{High-Energy Physics Institute, Tbilisi State University, 0186 Tbilisi, Georgia}

\author{A.~Magiera}
\affiliation{Marian Smoluchowski Institute of Physics, Jagiellonian University, 30348 Cracow, Poland}

\author{D.~Mchedlishvili}
\affiliation{High-Energy Physics Institute, Tbilisi State University, 0186 Tbilisi, Georgia}

\author{F.~M\"uller}
\affiliation{III. Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{N.N.~Nikolaev}
\affiliation{L.D. Landau Institute for Theoretical Physics, 142432 Chernogolovka, Russia}
\affiliation{Moscow Institute for Physics and Technology, 141700 Dolgoprudny, Russia}

\author{A.~Pesce}
\affiliation{University of Ferrara and INFN, 44100 Ferrara, Italy}

\author{V.~Poncza}
\affiliation{III. Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{F.~Rathmann}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{M.~Retzlaff}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{A.~Saleev}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{M.~Schm\"uhl}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{D.~Shergelashvili}
\affiliation{High-Energy Physics Institute, Tbilisi State University, 0186 Tbilisi, Georgia}

\author{V.~Shmakova}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}
\affiliation{Laboratory of Nuclear Problems, Joint Institute for Nuclear Research, 141980 Dubna, Russia}

\author{J.~Slim}
\affiliation{Institut f\"ur Hochfrequenztechnik, RWTH Aachen University, 52056 Aachen, Germany}

\author{A.~Stahl}
\affiliation{III. Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}

\author{E.~Stephenson}
\affiliation{Indiana University Center for Spacetime Symmetries, Bloomington,  Indiana 47405, USA}

\author{H.~Str\"oher}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}
\affiliation{JARA--FAME (Forces and Matter Experiments), Forschungszentrum J\"ulich and RWTH Aachen University, Germany}

\author{M.~Tabidze}
\affiliation{High-Energy Physics Institute, Tbilisi State University, 0186 Tbilisi, Georgia}

\author{G.~Tagliente}
\affiliation{Istituto Nazionale di Fisica Nucleare, 70125 Bari, Italy}

\author{R.~Talman}
\affiliation{Cornell University, Ithaca,  New York 14850, USA}

\author{Yu.~Uzikov}
\affiliation{Laboratory of Nuclear Problems, Joint Institute for Nuclear Research, 141980 Dubna, Russia}
\affiliation{Dubna State University, 141980 Dubna, Russia}
\affiliation{Department of Physics, M.V. Lomonosov Moscow State University, 119991 Moscow, Russia}

\author{Yu.~Valdau}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{A.~Wro\'{n}ska}
\affiliation{Marian Smoluchowski Institute of Physics, Jagiellonian University, 30348 Cracow, Poland}


\collaboration{JEDI collaboration}
\noaffiliation
